A numerical approach to the non-uniqueness problem of cosmic ray two-fluid equations at shocks

Cosmic rays (CRs) are frequently modeled as an additional fluid in hydrodynamic (HD) and magnetohydrodynamic (MHD) simulations of astrophysical flows. The standard CR two-fluid model is described in terms of three conservation laws (expressing conservation of mass, momentum and total energy) and one additional equation (for the CR pressure) that cannot be cast in a satisfactory conservative form. The presence of non-conservative terms with spatial derivatives in the model equations prevents a unique weak solution behind a shock. We investigate a number of methods for the numerical solution of the two-fluid equations and find that, in the presence of shock waves, the results generally depend on the numerical details (spatial reconstruction, time stepping, the CFL number, and the adopted discretization). All methods converge to a unique result if the energy partition between the thermal and non-thermal fluids at the shock is prescribed using a subgrid prescription. This highlights the non-uniqueness problem of the two-fluid equations at shocks. From our numerical investigations, we report a robust method for which the solutions are insensitive to the numerical details even in absence of a subgrid prescription, although we recommend a subgrid closure at shocks using results from kinetic theory. The subgrid closure is crucial for a reliable post-shock solution and also its impact on large scale flows because the shock microphysics that determines CR acceleration is not accurately captured in a fluid approximation. Critical test problems, limitations of fluid modeling, and future directions are discussed.

==> remove.tex <==
\begin{eqnarray}\label{eq:solwcrR}
\mathcal{R}^2\,\mathcal{A}- \mathcal{R}\, \mathcal{B}+ \mathcal{C}=0\, ,
\end{eqnarray} 
where
\begin{eqnarray}
\mathcal{A} &=& \left\{(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})\frac{\mathcal{M}^2_{\rm 1}}{2} +\frac{\gamma_{\rm g}}{\gamma_{\rm g}-1} + \frac{\gamma_{\rm cr}}{\gamma_{\rm cr}-1} \mathcal{P}_{\rm cr,1}   \right\}\\
\mathcal{B} &=& \left\{\frac{\gamma_{\rm g}}{\gamma_{\rm g}-1}(1-w_{\rm cr})+\frac{\gamma_{\rm cr}}{\gamma_{\rm cr}-1}w_{\rm cr}\right\}\nonumber \\ & & \left\{(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})\mathcal{M}^2_{\rm 1}+(1+\mathcal{P}_{\rm cr, 1})\right\}\\
\mathcal{C} & = & \left\{\frac{\gamma_{\rm g}}{\gamma_{\rm g}-1}(1-w_{\rm cr})+\frac{\gamma_{\rm cr}}{\gamma_{\rm cr}-1}w_{\rm cr} -\frac{1}{2}\right\}\nonumber \\ & &  \left\{(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})\mathcal{M}^2_{\rm 1}\right\} \  .
\end{eqnarray}
Here $w_{\rm cr}$ is a parameter specified in the downstream, and $\mathcal{P}_{\rm cr, 1}$ (Eq. \ref{eq:pcr1_nom}) and $\mathcal{M}_{\rm 1}(\mathcal{M}_{\rm cr, 1},\mathcal{M}_{\rm cr, 1})$ is upstream parameters. The solutions of Eq. (\ref{eq:solwcrR}) is given by
\begin{eqnarray}\label{eq:sol_wcrR}
\mathcal{R}_{\rm \pm}   = \frac{\mathcal{B}\pm (\mathcal{B}^2-4\mathcal{A}\mathcal{C})^{\HALF}}{2 \mathcal{A}} \ ,
\end{eqnarray}
Therefore, for a high Mach number flow, the shock compression ratio becomes



whose solutions can be written as $\mathcal{R}_{\rm \pm}$ Normalizing the gas and CR pressures w.r.t. the upstream gas pressure (as done previously) from Eq. (\ref{eq:pcr1}) we obtain
\begin{eqnarray}\label{eq:pcr2} 
\mathcal{P}_{\rm cr,2}&= & \epsilon_{\rm cr}\,\frac{\gamma_{\rm cr}-1}{\gamma_{\rm cr}} \mathcal{R}\left(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1}\right)\nonumber\\ & & \left\{\frac{\mathcal{M}_{\rm 1}^2}{2} + \frac{1}{\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1}}\left( \frac{\gamma_{\rm g}}{\gamma_{\rm g}-1} + \frac{\gamma_{\rm cr}}{\gamma_{\rm cr}-1} \mathcal{P}_{\rm cr,1}\right)\right\} .\nonumber \\
\end{eqnarray}
Using Eq. (\ref{eq:pcr2}), we substitute $\mathcal{P}_{\rm cr, 2}$ from Eq. (\ref{eq:mom_c2}) and (\ref{eq:engy_c2}), rearranging them we get
\begin{eqnarray} \label{eq:sol_ecrR}
\mathcal{R}^2\,\mathcal{A}- \mathcal{R}\, \mathcal{B}+ \mathcal{C}=0
\end{eqnarray}
where
\begin{eqnarray}
\mathcal{A} &=&(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})
\mathcal{M}^2_{\rm 1}\nonumber \\ & &\left\{\frac{\gamma-1}{2\gamma} - \frac{\gamma_{\rm cr}-1}{2\gamma_{\rm cr}}\epsilon_{\rm cr}\left(\frac{\gamma_{\rm g}-1}{\gamma_{\rm cr}-1}\frac{\gamma_{\rm cr}}{\gamma_{\rm g}}-1\right)\right\} \nonumber \\ & &+ 1 + \epsilon_{\rm cr}\left(\frac{\gamma_{\rm cr}-1}{\gamma_{\rm g}-1}\frac{\gamma_{\rm g}}{\gamma_{\rm cr}} - 1\right) \nonumber \\ & &
\mathcal{P}_{\rm cr,1} \left\{(1-\epsilon_{\rm cr})\left(\frac{\gamma_{\rm g}-1}{\gamma_{\rm cr}-1}\frac{\gamma_{\rm cr}}{\gamma_{\rm g}}\right)+\epsilon_{\rm cr}\right\}
\\
\mathcal{B} &=& \left\{(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})\mathcal{M}^2_{\rm 1}+(1+\mathcal{P}_{\rm cr, 1})\right\}\\
\mathcal{C} &=&  (\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1})\mathcal{M}^2_{\rm 1} \left(\frac{\gamma_{\rm g}+1}{2\gamma_{\rm g}}\right)
\end{eqnarray}
Therefore, the solutions can be obtained using Eq. (\ref{eq:sol_wcrR}). 


From Eq. (\ref{eq:wcr}), we note that the value of $w_{\rm cr}$ depends on the downstream CR and gas pressures. The CR pressure ($\mathcal{P}_{\rm cr,2}$) is already provided in Eq. (\ref{eq:pcr2}). The remaining quatity, $\mathcal{P}_{\rm g,2}$, can be obtained using  momentum conservation equation, Eq. (\ref{eq:mom_c2}) (one can also energy conservation equation, Eq. \ref{eq:engy_c2}, but both give an identical result) which gives
\begin{eqnarray}\label{eq:pg2}
\mathcal{P}_{\rm g, 2} = \left\{\left(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1}\right)\mathcal{M}_{\rm 1}^2\left(1-\frac{1}{\mathcal{R}}\right)+1+\mathcal{P}_{\rm cr,1}\right\} - \mathcal{P}_{\rm cr,2}
\end{eqnarray}
It is worth mentioning that the only constrain of the above equation is $\mathcal{P}_{\rm g, 2}> 0$, implying that the downstream CR pressure $\mathcal{P}_{\rm cr,2}< \left\{\left(\gamma_{\rm g} +\gamma_{\rm cr}\mathcal{P}_{\rm cr,1}\right)\mathcal{M}_{\rm 1}^2\left(1-\frac{1}{\mathcal{R}}\right)+1+\mathcal{P}_{\rm cr,1}\right\}$. From the values of  $\mathcal{P}_{\rm g,2}$ and $\mathcal{P}_{\rm cr,2}$, one can obtain $w_{\rm cr}$ as a function of $\mathcal{R}$, $\mathcal{M}_{\rm 1}$, $\mathcal{P}_{\rm cr, 1}$, and $\epsilon_{\rm cr}$ where $\mathcal{R}(\mathcal{P}_{\rm cr, 1}, \epsilon_{\rm cr})$ can be estimated from Eq. (\ref{eq:sol_ecrR}). Therefore, the parameter $w_{\rm cr}$ becomes a function of $\mathcal{M}_{\rm g, 1}$, $\mathcal{M}_{\rm cr, 1}$, and $\epsilon_{\rm cr}$.

